An Empirical Study on Benchmarks of Artificial Software Vulnerabilities

Recently, various techniques (e.g., fuzzing) have been developed for vulnerability detection. To evaluate those techniques, the community has been developing benchmarks of artificial vulnerabilities because of a shortage of ground-truth. However, people have concerns that such vulnerabilities cannot represent reality and may lead to unreliable and misleading results. Unfortunately, there lacks research on handling such concerns. In this work, to understand how close these benchmarks mirror reality, we perform an empirical study on three artificial vulnerability benchmarks - LAVA-M, Rode0day and CGC (2669 bugs) and various real-world memory-corruption vulnerabilities (80 CVEs). Furthermore, we propose a model to depict the properties of memory-corruption vulnerabilities. Following this model, we conduct intensive experiments and data analyses. Our analytic results reveal that while artificial benchmarks attempt to approach the real world, they still significantly differ from reality. Based on the findings, we propose a set of strategies to improve the quality of artificial benchmarks.

==> prev/0-abstract.tex <==
\begin{abstract}
In recent years, dozens of techniques (e.g., fuzzing) have been developed 
to find vulnerabilities in software systems. To comprehensively 
measure the effectiveness of those techniques and understand their 
limitations, the community has been developing benchmarks of 
artificial vulnerabilities because of a shortage of ground-truth. However, we find the bug finding tools that perform well on artificial benchmarks may not perform well in real-world vulnerabilities.
So people have wide doubts about 
the validity of those artificial benchmarks, mainly concerning that
such vulnerabilities cannot represent the reality and they could 
lead to unreliable and misleading results of the bug finding techniques. 
Unfortunately, there lacks research on handling such concerns. 

In this work, aiming to understand how close these benchmarks mirror the reality and whether they can measure the effectiveness of vulnerability detection tools, we perform a systematic empirical study on three most-used artificial vulnerability benchmarks - LAVA-M, Rode0day and CGC (2669 bugs in total) and a wide range of real-world memory corruption vulnerabilities (80 CVEs in total).
Furthermore, we propose a general model to depict the properties of memory corruption vulnerabilities, together with how the properties influence the evaluation of the vulnerability detection tools. 
Following this model, we make a carefully controlled workflow to carry out analytic experiments with 800 man-hours spent.  
Our analytic results reveal that while artificial 
benchmarks attempt to approach the real world, they still 
significantly differ from the reality in terms of the program properties, bug requirements and vulnerability types.
% To further support our study,
% we modify LAVA-M according to our conclusions and evaluate the influences
% that such differences bring to the vulnerability detection tools.
% Aiming at making artificial benchmarks 
% more realistic and better to measure the vulnerability detection tools, 
Last but not least, we modify LAVA-M and propose a set of strategies from the program and vulnerability perspectives to make the artificial vulnerabilities closer to their real-world counterparts. 
% the program perspective (eg. increasing LOC and CCN of the benchmarks), and 
% the vulnerability perspective (eg. adding data transformation along the execution trace).

\end{abstract}

==> prev/1-introduction.tex <==
\section{Introduction}

Software vulnerability has long been a fundamental threat against 
computer security. To alleviate this situation, tremendous research
has been conducted on developing techniques to find software 
vulnerabilities. In the last five years, over 60 papers about 
vulnerability detection have been published on top conferences 
of cyber security and software engineering~\cite{klees2018evaluating}.

To comprehensively measure the utility and understand the limitations 
of techniques of vulnerability detection, the community has been developing 
artificial benchmarks of software vulnerabilities. People compose 
such benchmarks by either injecting vulnerabilities into 
existing programs~\cite{dolan2016lava,Rode0dayWeb} or crafting 
artificial vulnerable programs~\cite{CGCWeb}. Compared with benchmarks 
consisting of real-world programs, artificial benchmarks have two 
advantages. On the one hand, artificial benchmarks can provide 
ground truth of vulnerabilities, which is essential 
for the evaluation of vulnerability coverage. On the other hand, 
artificial benchmarks can easily synthesize different types of diversities, 
such as diversities in the programs and diversities around the 
vulnerabilities. Such diversities are important in evaluating the 
generality of vulnerability detection techniques. 




Despite the above advantages, while these bug finding tools  perform well on artificial benchmarks, they may not perform  well in real-world programs. For example, Wang et al.\cite{WangXLC2020TGF} find that although Angora (a new mutation-based fuzzer) can detect almost all the bugs that inserted by LAVA while AFL performs worse, AFL can discover 62\% more vulnerabilities (e.g., CVE-2017-6966, CVE-2018-11416, CVE-2017-13741) than Angora within 24 hours across 8 runs.
So researchers are hesitating 
with adopting artificial vulnerability benchmarks, concerning that 
these benchmarks insufficiently represent the reality and thus,  
evaluation using such benchmarks is unreliable or even 
misleading. Unfortunately, there lacks research on handling such 
concerns in the literature. 

In this work, we aim to understand the validity of artificial 
benchmarks. Our methodology is to compare the mainstream benchmarks of 
artificial vulnerabilities (LAVA-M~\cite{dolan2016lava}, 
Rode0day~\cite{Rode0dayWeb} and CGC~\cite{CGCWeb}, 2669 artificial bugs in total) with real-world 
vulnerabilities (80 CVEs in total). 
%From external to essential, the properties of the program itself, like \textbf{program volume (lines of code (LOC), cyclomatic complexity (CCN))} and \textbf{functionality diversity} can affect the evaluation of vulnerability detection tools such as generality and scalability.
%The different requirements to form vulnerabilities, like \textbf{reaching the buggy locations} and \textbf{triggering the specific states}, can influence program state coverage and sensitivity of tools.
%Also, the kinds of unexpected behaviours (vulnerability types) can affect the sensitivity of tools.
%
% Centering around above aspects, we focus on the following questions and 
% seek answers through our study:\\
Centering around the major
aspects that may cause differences between artificial benchmarks and real-world vulnerabilities,
we focus on the following questions and seek answers through
our study:\\
{\bf Q1.} \emph{How do the 
programs in artificial benchmarks differ from the programs containing real-world 
vulnerabilities?}\\ %Properties of the benchmark programs, such as code size 
%and functionality complexity, can have large impacts on the effectiveness 
%and efficiency of vulnerability finding. This motivates us to perform 
%a comparison from the point view of the programs.\\
{\bf Q2.} \emph{How do artificial vulnerabilities differ from real-world
vulnerabilities? Can artificial vulnerabilities sufficiently mirror 
the reality?} \\
%Needless to say, properties related to vulnerabilities are the 
%most important factors that artificial benchmarks need to consider. 
%Benchmarks containing vulnerabilities that deviate from the real-world 
%will be less useful. Therefore, our study emphasize on this aspect
%{\jun This is a little bit bluffing. Please concretize}
{\bf Q3.} \emph{What improvements can we make towards more realistic 
artificial vulnerabilities benchmarks?} 
%By understanding how artificial benchmarks
%deviate from the reality, we also aim to explore potential directions 
%towards improvements. 


To systematically answer the above questions, we develop a general model that captures the essential properties of programs and vulnerabilities that can help our analysis.
This model depicts the properties of memory corruption vulnerabilities, together with how the properties influence the evaluation on the vulnerability detection tools, as we will detail in Section~\ref{sec:model}. 
Following this model, we carry out our experiments and summarize answers to the above three questions. 
In short, our study reveals that while artificial benchmarks attempt to approach the real world, they still differ from the reality.
For \textbf{Q1}, we found that not all of the evaluated benchmarks are close to real world in the complexity of the program's control flow.
For \textbf{Q2}, we found that the artificial benchmarks created by injecting bugs are faced with the problem of not capturing the key properties of real-world vulnerabilities.
For \textbf{Q3}, we propose several strategies to make artificial benchmarks more realistic based on our analyses and experiments.
% For \textbf{Q1}, artificial benchmarks, especially CGC, tend to include programs that are simpler than the 
% real programs, such as smaller \emph{program volume} (lines of code (LOC), cyclomatic complexity (CCN)) and less \emph{functionality diversity}. 
% And the program properties can influence the \emph{generality} and \emph{scalability} of vulnerability detection tools.
% 
% {\jun The following paragraph is not readable. Please re-phrase}
% With regard to \textbf{Q2}, artificial vulnerabilities typically have less complex triggering 
% conditions (namely \emph{bug requirements}) in control flow and data flow than real-world vulnerabilities. 
% As to artificial benchmarks of vulnerabilities, the types of magic bytes comparisons are single.
% The difficulty of path conditions lack even distribution and there is a hard-to-match magic number by the end of the path.
% The input data does not go through data transformations and match the magic bytes directly. 
% What's more, there are not special states as a prerequisite for triggering the artificial vulnerabilities. 
% The above features of artificial vulnerabilities can not better represent the real-world cases and measure the \emph{program state coverage} of tools well.
% Also, the single vulnerability type (namely \emph{unexpected behaviours}) of artificial vulnerabilities, such as only buffer overflow can not evaluate the \emph{sensitivity} of tools. 
% All of the categories of differences that Q1 and Q2 mentioned can lead to overrating of vulnerability detection techniques. 
% To further learn how these differences affect the detection tools, we conduct a series of comparison experiments according to the features of the real world.
% The results of the experiments show that the artificial bugs cannot mirror the reality well because they may not fairly reflect the properties of the vulnerability detection tool.
% 
% For \textbf{Q3}, towards offsetting those differences and making the existing artificial benchmarks more 
% realistic, we also propose a set of improving strategies and the details of three research questions 
% can be found in Section~\ref{sec:analysis_results}.

In summary, our major contributions are four-fold as follows.
\begin{itemize}
    \item First, to the best of our knowledge, we perform the first in-depth empirical study on the analysis of benchmarks of artificial vulnerabilities with manually verifies and confirms. 
    Our large-scale analysis covers 2669 artificial bugs and 80 real-world vulnerabilities (CVEs), which is the most comprehensive comparison between artificial vulnerabilities and real-world ones.
    \item Second, we develop a general model to describe essential software vulnerabilities, together with how the program properties and bug requirements influence the evaluation on the vulnerability detection tools. 
    % Following this model, we carry out our analytic experiments. 
    \item Third, our results provide quantitative evidence on the differences between artificial and real-world vulnerabilities from the properties of the program itself and the control-flow and data-flow requirements to trigger a vulnerability. 
    We also identify the factors that how they influence the evaluation of vulnerability detection techniques. 
    \item Fourth, we modify the benchmark according to what we have observed on control flow and data flow. 
    The results of experiments show that our modifications confirm our findings and evaluate the vulnerability detection tools well in the four properties.
    We also propose new improvements toward making artificial benchmarks more realistic.
\end{itemize}


% The rest of this paper is organized as follows.
% Section~\ref{section:Background} 
% introduce background and our motivation.
% Section~\ref{sec:model}
% describes the general model we propose. 
% Then we explain the methodology and datasets of our experiments in Section~\ref{section:DATASETS AND METHODOLOGY}. Section~\ref{sec:analysis_results} 
% presents our findings and our answers to the above three 
% research questions. Section~\ref{sec:related} summarizes related
% works and section~\ref{sec:conclusion} concludes this paper. 



% LAVA-M and Rode0day do not have an even distribution of difficulty in solving if-conditions, especially harder noticeably in the last constraint solving.
% Also, the type of magic number in the paths is almost 32-bit, which is different from the reality in types and proportions.
% What's more, the bugs inserted by LAVA and Rode0day can be triggered successfully once the last magic number is solved out without satisfying some specific value, which is distinct from the true circumstances {\jun This is unclear. I am not sure I get it}. 
% The values of magic numbers are often the direct copies of inputs without any data transformation, which is different from real world.


==> prev/2-threats-to-validity.tex <==
\section{Threats to Validity}

There are some potential threats to the validity of this study.
Foremost is simply the representative of all memory corruption vulnerabilities in real world.
We believe, however, that we have chosen a representative set of real-world vulnerabilities and we will argue from three aspects.

\textbf{Vulnerability Type.}
The first potential threat is the limited scope of the study in terms of the vulnerability types. 
In this paper, we focus on the memory corruption vulnerabilities
as they have been ranked among the most dangerous software errors~\cite{CWEdanger} due to their high severity and real-world impact~\cite{ms_mc}.
There are more than 10,000 memory corruption vulnerabilities listed on the CVE website. We crawled the pages of the current 95K+ entries (2001-2017) and analyzed their severity scores (CVSS). 
Our result shows that the average CVSS score for memory corruption vulnerabilities is 7.6, which is clearly higher than the overall average (6.2), confirming their severity.

Additionally, the majority of vulnerabilities in the artificial benchmarks to be studied (LAVA-M, CGC and Rode0day) are in types of memory corruptions.
Testing memory corruption vulnerabilities in both artificial benchmarks and real world, we can make a more fair comparison. 
We believe that the vulnerability type we have chosen is well-founded, and the research results will be applicable to other types of vulnerabilities as well.


\textbf{Justifications on the Dataset Size.}
The second potential threat to validity is that the size of our dataset, specifically the number of real-world vulnerabilities.
We select 80 CVEs as real-world vulnerabilities and argue that the size of our dataset is reasonably large.
For example, recent work that uses vulnerabilities in the CVE list to evaluate their vulnerability detection systems are limited to less than 10 vulnerabilities~\cite{carlini2015control, hu2016data, castro2006securing, akritidis2008preventing}, due to the significant manual efforts needed to build ground truth data.

Also, it should be noted that reproducing and analyzing the vulnerabilities are extremely difficult and took us a lot of manpower(e.g., triggering and analyzing the crash step by step) are different for each case, and thus cannot be automated.
Our experiments demanded 800 man-hours to finish, covering a dataset of 80 CVE cases randomly sampled from those reported in the last 15 years. 
So considering both the number and manual efforts, we believe the size of dataset is enough. 


\textbf{Creation of the dataset.}
We obtained the real-world vulnerability types from the CVE entry's description or its references, which is shown in Table~\ref{tab:CGC-Realworld-Bug-Type}, and the percentage of every category of memory corruption vulnerabilities in our dataset nearly follows the statistics we collect from the real world. 
To make the real-world vulnerabilities more extensive and the analytic results more general, we divide the vulnerabilities into 5 times bins(3 - year period) whose over-time trend of our dataset relatively consistent with that of the entire CVE dataset~\cite{CVEdatabase}.
Also, our real-world programs cover 80 representative CVEs~\cite{CVEWeb}, which are from 40 different open-source software products (eg. {\tt ngnix}, {\tt openjpeg}, {\tt perl}, {\tt php}) and a diverse set of memory corruption vulnerabilities, 9 categories in total.
To sum up, the creation of the dataset is consist with the 
aforementioned aspects and the real-world circumstances, 
hence the dataset is of rationality and representativeness.
The 80 real-world vulnerabilities with CVE-IDs are shown in Table~\ref{tab:CVE-ID}, and the concrete methodology will be introduced in detail in Section~\ref{section:DATASETS AND METHODOLOGY}.



==> prev/3-background-and-motivations.tex <==
\section{Background and Motivations}

\label{section:Background}





In this section, we start by introducing the background of security vulnerabilities and benchmarks we study.
We then proceed to describe our research goals.

% \subsection{CVE}
% {\jun This needs to be re-orged. I could not parse it}
% The Common Vulnerabilities and Exposures (CVE) system provides a reference-method for publicly known information-security {\jun ???} vulnerabilities and exposures.
% When software users identify a vulnerability, they can request a CVE ID from CVE Numbering Authorities.
% CVEs are for software that has been publicly released and intended for use with respect to identifying vulnerabilities~\cite{CVE}.
% Need to note that the real-world vulnerabilities in our datasets are from the CVE website~\cite{CVEWeb}, and we focus on the memory corruption vulnerabilities.

% \begin{figure}[b]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figs/lava_overview_alt2.pdf}
% 	\caption{An overview of how LAVA plants bugs.}
% 	\label{fig:LavaOverview}   
% \end{figure}


\subsection{Memory Corruption Vulnerability}

A memory corruption vulnerability is a security vulnerability that allows attackers to manipulate in-memory content to crash a program or obtain unauthorized access to a system.
Memory corruption vulnerabilities such as "Buffer-Overflow", "Null-Pointer-Dereference" and "Use-After-Free", have been ranked among the most dangerous software errors~\cite{CWEdanger}.
% A recent example is the vulnerability exploited by the {\tt WannaCry} cryptoworm (CVE-2017-0144) which shut down 300,000+ servers.
% Our study focuses on memory corruption vulnerabilities due to their high severity and real-world impact~\cite{ms_mc}.







\subsection{Benchmarks of Artificial Software Vulnerabilities}
\label{sec:dataset_bg}

\begin{figure}[hb]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/lava_overview_alt2.pdf}
	\caption{An overview of how LAVA plants bugs.}
	\label{fig:LavaOverview}   
\end{figure}


In spite of decades of research in bug detection tools, there is a surprising dearth of ground-truth corpora that can be used to evaluate the efficacy of such tools.
The lack of ground-truth datasets means that it is difficult to perform large-scale studies of bug discovery.
Because for statistically meaningful evaluation, the security vulnerabilities are spread too thin and do not expose all facets of the underlying problem~\cite{pewny2016evilcoder}.




To comprehensively measure the utility and understand the limitations of vulnerability detection techniques, the community has been developing artificial benchmarks of vulnerabilities.  
In recent years, three widely-used artificial vulnerability databases have sought to address the need for ground-truth benchmark and there are two categories of them. 
\textbf{LAVA-M} and \textbf{Rode0day} inject large numbers of bugs into program source code automatically and include similar bugs structurally.
And \textbf{DARPA Cyber Grand Challenge} (CGC) contains a series of fairly small programs with known bugs written by security experts.
In this part, we will briefly provide background information on the artificial vulnerabilities before introducing our study.


LAVA is a prevalent ground-truth corpus generator, which can efficiently and automatically add memory corruption bugs into C/C++ programs on demand. 
LAVA currently concentrates on injecting Buffer-Overflow bugs and produces corresponding proof-of-concept inputs as their triggers~\cite{dolan2016lava}.



Figure~\ref{fig:LavaOverview} presents an overview of LAVA. 
When LAVA obtains the source code and series of input files of the program, it finds unused portions of the input by running the program with dynamic taint analysis~\cite{newsome2005dynamic} on each specific input.
This data parts of the inputs bytes are \emph{dead} (i.e., it does not influence control flow), \emph{uncomplicated} (not modified), and \emph{available}, namely DUAs. 
Since DUAs are often a direct copy of input bytes and can be set to any chosen value without sending the program along a different path, LAVA intends to regard them as candidate triggers for memory corruption. 
At the DUA site, code is inserted to copy the DUA's value into a global variable via a call to {\tt lava\_set}.
Then LAVA finds potential attack points (ATPs), which is a program instruction involving a memory read or write whose pointer can be modified and must occur temporally after a DUA along the program execution.
LAVA introduces a dataflow relationship between DUA and ATP along the trace by modifying the source code as follows and at the attack point, {\tt lava\_get} retrieves the value, compares it to the trigger value (magic number).
A memory corruption occurs if the condition is met.



% \begin{enumerate}
%  \item At the DUA site, code is inserted to copy the DUA's value into a global variable via a call to {\tt lava\_set}.
%  \item At the attack point, {\tt lava\_get} retrieves the value, compares it to the trigger value (magic number).
%  \item If the condition is met, adds the DUA to the attacked pointer in order to cause a memory corruption.
% \end{enumerate}


\textbf{LAVA-M}, which generated by LAVA, is one of our datasets in our study. It is a benchmark of artificial software vulnerabilities that injected more than one bug at a time into the source code and used widely to evaluate vulnerability detection tools.

\textbf{Rode0day}~\cite{Rode0dayWeb} is a recurring bug finding contest, which is also a benchmark to evaluate vulnerability discovery techniques. Evolved from LAVA, Rode0day challenges are all standard 32-bit Linux ELF files using automated bug insertion to generate a new corpus of buggy programs. 
%Based on technology of LAVA, Rode0day makes some changes, such as modifies the data flow between DUAs and attack points and add a compile-time flag to the modified C-source files that can produce versions of the binaries that logged to standard output whenever a DUA guard was successfully triggered, which can easily determine which bug a competitor triggered when an input causes a crash.


\textbf{CGC}~\cite{CGCWeb}, a competition among autonomous vulnerability analysis systems, is a widely adopted benchmark in recent studies~\cite{chen2018angora,li2017steelix,rawat2017vuzzer,zhao2019send}.
This competition resulted in a collection of small programs with known vulnerabilities and triggering inputs.
Each challenge of CGC contains one or more bugs, which are deliberately devised by security experts to evaluate vulnerability detection tools.



\subsection{Motivations}

While existing works focus on proposing new benchmarks that can be used to evaluate the efficacy of vulnerability detection tools~\cite{roy2018bug, dolan2016lava, Rode0dayWeb, CGCWeb, pewny2016evilcoder}, there is a lack of systematic understanding of whether the artificial vulnerabilities can represent the real-world vulnerabilities.
Although other works suggest that some widely-used benchmarks, like LAVA-M, Rode0day and CGC are different from real-world bugs in several ways~\cite{roy2018bug, hu2018chaff, pewny2016evilcoder}, they did not provide in-depth analysis of the benchmarks.
Moreover, there is also an absence of analysis on how the different properties of the benchmark vulnerabilities can reflect the different features of the vulnerability detection tools.
Also, analyzing the differences between artificial and real-world vulnerabilities can help to create more realistic benchmarks for tool evaluation.
Thus, we propose a study to provide a first in-depth understanding of similarities and differences between artificial and real-world vulnerabilities while exploring solutions to make artificial bugs more realistic.




% If the bugs created artificially are so far different from naturally occurring bugs, they can lead to misleading results to evaluate the efficacy of vulnerability detection tools.
% Understanding the different aspects of artificial and real-world vulnerabilities is a prerequisite step when creating a more realistic benchmark and evaluating the tools.
% Although other works suggest that some widely-used benchmarks, like LAVA-M, Rode0day and CGC are different from real-world bugs in a number of ways~\cite{roy2018bug, hu2018chaff, pewny2016evilcoder}, they did not provide in depth analysis of the benchmarks.
% Although other works suggest that some widely-used benchmarks, like LAVA-M, Rode0day and CGC are so far different from real-world bugs in a number of ways~\cite{roy2018bug} and may not evaluate vulnerability detection tools well~\cite{hu2018chaff, pewny2016evilcoder}, they do not analyze the benchmarks more comprehensively.
% Using the memory corruption vulnerabilities as examples, our study seeks to provide a first in-depth understanding of similarities and differences between artificial and real-world vulnerabilities while exploring solutions to make artificial bugs more realistic.






==> prev/4-model-overview.tex <==
\section{Model Overview}
\label{sec:model}

\begin{figure*}[h]
	\centering
	\includegraphics[width=\textwidth]{figs/model_new_2.pdf}
	\caption{The model for memory corruption vulnerability and vulnerability detection tool.}
	\label{fig:model}   
\end{figure*}

In this paper, we focus on the memory corruption vulnerability, which is the majority of software security defects~\cite{ms_mc}.
Instead of discussing the vulnerabilities case by case, we propose a \emph{general model} to describe the memory corruption vulnerabilities by summarizing the \emph{properties of the vulnerable program} and the \emph{requirements for triggering the vulnerability}.
Besides the model for vulnerabilities, we also propose a model to represent the different \emph{features of the vulnerability detection tool} and how they are \emph{affected by} the components of the vulnerability model.
This is because the goal of the benchmarks is to evaluate the vulnerability detection tools.
So we further extend the vulnerability model by adding the relations with the properties of the vulnerability detection tool.
Figure~\ref{fig:model} depicts our model, in which the cyan boxes represent the main components of a bug, while the pink boxes represent the major properties for triggering unexpected behaviours of the program and the gray boxes are the desired properties of the vulnerability detection tools.
This model provides a systematic basis for our experiments and analyses.
Here we discuss the model in detail.
% Aiming to systemically investigate how close the bugs in benchmarks mirror the reality, we need to have a deep look into the characteristics of causing memory corruption vulnerabilities.
% To make our summary universal for each memory corruption vulnerability, we make a generalization of the requirements to trigger a vulnerability and propose a high-level vulnerability model rather than studying bugs case by case.
% Note that, we focus on memory corruption vulnerabilities in this paper since such a category of vulnerabilities has become the majority of the security defects~\cite{ms_mc}.

% Moreover, because the goal of the artificial benchmarks is to evaluate different properties of vulnerability detection tools, this model also demonstrates the desired properties for tools in the gray boxes and how they are connected with the different components in the model.

From Figure~\ref{fig:model}, we can see that a typical memory corruption vulnerability happens like this: first, the target program is fed with a malicious input; then, the program must contain bugs/vulnerabilities which can be triggered by the malicious input; last, after the vulnerability is triggered successfully, the program will behave unexpectedly.

Triggering the unexpected behaviour is the coaction of the malicious input and the vulnerability inside the program.
In our model, we focus on the requirements for the program to become vulnerable.
Such requirements are called \textbf{bug requirements} in our model.
The bug requirements can be summarized as follows.
To trigger the vulnerability, we need to feed a specific input to the buggy program.
This input can be in different forms, such as a file, a series of user actions or a stream of data, but it should satisfy the following two conditions.
\ding{182} By executing this input, the control flow must \textbf{reach the buggy location} in the program.
Nevertheless, the reachability problem is hindering the detection of most vulnerabilities.
For example, the control flow needs to go through a series of complex conditions and the data flow needs to go through a series of data transformations.
\ding{183} In further, this input may have to lead the program's execution to the location with \textbf{a specific program state}.
In other words, only reaching the buggy location is \emph{not} enough.
For example, for a Use-After-Free vulnerability, the program may have reached the location of the buggy ``\emph{use}" without passing through the corresponding ``\emph{free}".
In this case, the vulnerability is not triggered.
To trigger the Use-After-Free vulnerability, the program must reach the ``\emph{use}" from the path where the ``\emph{free}" has been called.
To summarize, a vulnerability is triggered when the buggy program is fed with an input that can help to reach the buggy location with a specific program state.


% Besides the bug requirements, we take the properties of buggy programs into consideration because the depth of vulnerability and difficulty of insertion can be influenced by the program inherent natures~\cite{roy2018bug}.
Besides the bug requirements, the properties of the buggy programs can also affect the performance of the vulnerability detection tools on these programs~\cite{roy2018bug}.
For example, \textbf{program volume} refers to the software metric used to measure the internal characteristics of a computer program, including lines of code (LOC)\scarlett{loc may not needed}, cyclomatic complexity (CCN), etc.

% And our study focus on the two aspects of the program properties.

After triggering the vulnerability, the buggy program will \textbf{behave unexpectedly} in different ways.
The program may run into Buffer-Overflow, Null-Pointer-Dereference, Use-After-Free, etc. and harm the software and system.

Since the goal of the artificial benchmarks is to evaluate different
properties of vulnerability detection tools, our model also shows how the different components of vulnerabilities are connected with the properties of tools.
To be specific, if the benchmarks contain larger and more complex programs, it can better evaluate whether the tools are scalable enough from the success rate in those programs. 
So program volume is related to the \emph{scalability} of the vulnerability detection tool.
% If the programs in benchmarks own a diversity of functionalities, it can better evaluate the \emph{generality} of the detection techniques to determine whether they can handle different application scenarios.
% Thus functionality diversity has a close connection with generality. 
Both reaching the buggy location and triggering specific states require the tool to use some strategies to solve the control-flow and data-flow constraints to have a larger \emph{program state coverage}.
Last but not least, some unexpected behaviours of the buggy programs require the tool to be sensitive enough to detect.
So the vulnerability types can evaluate the \emph{sensitivity} of tools.


To sum up, the high-level model contains the above properties mentioned and forms the basis of our study. 
The properties of buggy programs are related to \emph{Q1}, and the bug requirements are related to \emph{Q2}.
Following the general model, we design our information extraction methodology in Section~\ref{section:DATASETS AND METHODOLOGY} and discuss the details of three research questions in Section~\ref{sec:analysis_results}.



% The analysis of properties of buggy programs is 
% and answer the aforementioned three research questions in Section~\ref{sec:analysis_results}.
 

% This model forms the basis of our study.
% Following the model, we design our information extraction methodology, manually collect and analyze 2749 bugs totally, and finally answer three research questions.








==> prev/5-methodology-dataset.tex <==
\section{Datasets and Methodology}

\label{section:DATASETS AND METHODOLOGY}

% Aiming to detect the similarity between real-world vulnerabilities and benchmarks, we choose the widely-used LAVA, DARPA Cyber Grand Challenge (CGC), and Rode0day as the representative benchmarks in our study. 

In this section, we describe the dataset for our experiments and high-level information extraction methodology.


\subsection{Datasets}
\label{sec:datasets}

\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{3mm}{
\caption{Dataset overview.}
\label{tab:dataset-overview}
\begin{tabular}{c|c|c}
\toprule[1.3pt]
\textbf{Dataset}  & \textbf{Bugs Number} & \textbf{Programs Number} \\ \hline
\textbf{Real World}      & 80                   & 40                               \\ 
\textbf{CGC}      & 119                  & 93                              \\ 
\textbf{LAVA-M}   & 587                  & 4                                \\ 
\textbf{Rode0day} & 1963                 & 9                                \\ \hline
\textbf{Total}    & 2749                 & 146                               \\ 
\bottomrule[1.3pt]
\end{tabular}}

\end{table}


\textbf{Artificial Benchmarks.}
We choose three widely-used artificial benchmarks, which are LAVA-M, Rode0day and CGC. 
LAVA-M and Rode0day inject bugs into programs automatically.
We collect 587 bugs in LAVA-M and 1963 bugs in Rode0day.
And LAVA-M insert bugs into 4 software programs ({\tt base64}, {\tt md5sum}, {\tt uniq} and {\tt who}) while Rode0day insert bugs into 9 programs.
For CGC, the specialist-written benchmark, we select 93 challenges with 119 memory corruption bugs (Table~\ref{tab:dataset-overview}).


% \begin{figure}[htbp]
% \centering
% \begin{minipage}[t]{0.24\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/Vulnerability_Type.pdf}
% \caption{Vulnerability Type.}
% \label{fig:Vulnerability-type}
% \end{minipage}
% \begin{minipage}[t]{0.24\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figs/of-vulnerability-over-time.pdf}
% \caption{\# of Vulnerabilities Over Time.}
% \label{fig:of-vulnerability-over-time}  
% \end{minipage}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \begin{minipage}{0.435\linewidth}
% \includegraphics[width=\linewidth,height=1.2in]{figs/Vulnerability_Type}
% \vspace{-0.2in}
% \caption{Real-world vulnerability type of our dataset.}
% \label{fig:Vulnerability-type}
% \vspace{-0.03in}
% \end{minipage}
% \hfill
% \begin{minipage}{0.45\linewidth}
%  \includegraphics[width=\linewidth,height=1in]{figs/of-vulnerability-over-time}
% \vspace{-0.2in}
% \caption{Real-world vulnerabilities of our dataset over time.}
% \label{fig:of-vulnerability-over-time}
% \vspace{-0.03in}
% \end{minipage}
% %\caption{\fixme{XXX}}
% %\label{fig:v_type_year}
% \end{figure}





\textbf{Real-world programs.}
We analyze 80 representative CVEs~\cite{CVEWeb} which are from 40 different open-source software products (eg. {\tt ngnix}, {\tt openjpeg}, {\tt perl}, {\tt php}).
The reason that we focus on memory corruption vulnerabilities due to their high severity and significant real-world impact.
% The 80 real-world vulnerabilities with CVE-IDs are shown in Table~\ref{tab:CVE-ID}.
We list the CVE-IDs of 80 real-word vulnerabilities in Appendix~\ref{apendix:cve_ids}
% Figure~\ref{fig:of-vulnerability-over-time} shows the number of real-world vulnerabilities we collect in different years.
% We divide the vulnerabilities into 5 times bins (3-year period).
% Not only is this over-time trend of our dataset relatively consistent with that of the entire CVE database~\cite{CVEdatabase} but also we can obtain some more general analytic results during the research.
% Our real-world programs cover a diverse set of memory corruption vulnerabilities, 9 categories in total as shown in Figure~\ref{fig:Vulnerability-type}.
We obtained the types from the CVE entry's description or its references.
Note that, the percentage of every category of memory corruption
vulnerabilities nearly follows the statistics we collect from
the real world, which is shown in Table~\ref{tab:CGC-Realworld-Bug-Type}.
 


% \subsection{Datasets Background}
% \label{sec:dataset_bg}

% \textbf{LAVA} is a prevalent ground-truth corpus generator, which can efficiently and automatically add memory corruption bugs into C/C++ programs on demand. 
% In this way, it creates a huge bug corpus for tool developers and enables rigorous tool evaluation. 
% LAVA currently concentrates on injecting out-of-bounds reading and writing bugs and produces corresponding proof-of-concept inputs as their triggers, rather than the actual exploits~\cite{dolan2016lava}.

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figs/lava_overview_alt2.pdf}
% 	\caption{An overview of how LAVA plants bugs.}
% 	\label{fig:LavaOverview}   
% \end{figure}

% Figure~\ref{fig:LavaOverview} presents an overview of LAVA. When LAVA obtains a program source and its series of input files, it finds unused portions of the input by running the program with dynamic taint analysis~\cite{newsome2005dynamic} on each specific input.
% This data parts of the inputs bytes are \emph{dead} (i.e., it does not influence control flow), \emph{uncomplicated} (not modified), and \emph{available}, namely \textbf{DUAs}. 
% Since DUAs are often a direct copy of input bytes and can be set to any chosen value without sending the program along a different path, LAVA intends to regard them as candidate triggers for memory corruption. 
% Then LAVA finds potential attack points temporally after a DUA and introduces a dataflow relationship between DUA and the attack point along the trace to actually trigger the bug. 

% LAVA-M is a benchmark of artificial software vulnerabilities that injected more than one bug at a time into the source code and used widely to evaluate vulnerability detection tools. 


% \textbf{Rode0day}~\cite{Rode0dayWeb} is a recurring bug finding contest, which is also a benchmark to evaluate vulnerability discovery techniques. Evolved from LAVA, Rode0day challenges are all standard 32-bit Linux ELF files using automated bug insertion to generate a new corpus of buggy programs. 
%Based on technology of LAVA, Rode0day makes some changes, such as modifies the data flow between DUAs and attack points and add a compile-time flag to the modified C-source files that can produce versions of the binaries that logged to standard output whenever a DUA guard was successfully triggered, which can easily determine which bug a competitor triggered when an input causes a crash.


% \textbf{CGC}~\cite{CGCWeb}, a competition among autonomous vulnerability analysis systems, is a widely adopted dataset in recent studies~\cite{chen2018angora,li2017steelix,rawat2017vuzzer,zhao2019send}.
% CGC contains the 248 challenges with 296 binary programs~\cite{peng2018t}, which are deliberately devised by security experts to evaluate vulnerability detection tools. 

% \begin{figure*}[!ht]
% \centering
% \begin{minipage}{0.45\linewidth}
%  \includegraphics[width=\linewidth,height=1.2in]{figs/An-example-of-codecoverage-report}
% \vspace{-0.2in}
% \caption{An example of code coverage report generated by LCOV in {\tt base64} of LAVA-M.}
% \label{fig:report}
% \vspace{-0.03in}
% \end{minipage}
% \hfill
% \begin{minipage}{0.435\linewidth}
%  \includegraphics[width=\linewidth,height=1.2in]{figs/An-example-of-codecoverage-in-base64-of-lava-m}
% \vspace{-0.2in}
% \caption{An example of program execution in {\tt base64} of LAVA-M.}
% \label{fig:code-coverage-example}
% \vspace{-0.03in}
% \end{minipage}
% %\caption{\fixme{XXX}}
% %\label{fig:v_type_year}
% \end{figure*}

\subsection{Methodology}
\label{sec:methodology}

We use different tools to collect the necessary data for analysis.
The overall workflow for our data collection is shown in Figure~\ref{fig:workflow}.
As described in the workflow, we need to collect two different types of data for answering the research questions.
First, we need to extract the inherited data from the programs (the \textit{extracted information} in Figure~\ref{fig:workflow}).
Second, we need to extract the execution trace of the vulnerabilities/bugs (the \textit{code execution trace} in Figure~\ref{fig:workflow}).


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/workflow_alt1.pdf}
	\caption{Workflow of the analyses of benchmarks and real-world vulnerabilities.}
	\label{fig:workflow}   
\end{figure}




% To compare the artificial software vulnerabilities with real-world ones, we need to collect the features of them, which are mentioned in the research question and the model above.
% To be specific, the inherent natures of buggy programs themselves and the bug requirements, as is shown in the model above. 
% Thus, we design a workflow as Figure~\ref{fig:workflow} to analyze the datasets. 

% \yunlan{When we determine where to put code coverage and function coverage, check the sequence in workflow here.}
To answer \textbf{Q1}, we need to get the cyclomatic complexity (CCN) of the program.
We write \texttt{python} scripts based on the lizard~\cite{lizard} library to obtain the CCN of the target program.
% We run commands in the libraries of {\tt python} to obtain the LOC and CCN.
Combining automatic collection and manual analysis, we can obtain the cyclomatic complexity and unexpected behaviours of the programs.


To answer \textbf{Q2}, we need a deeper look into how the vulnerabilities occur and the conditions for reaching the buggy locations and triggering the specific states.
Thus, we need to collect the \emph{execution trace} of the vulnerability.
For this purpose, we need to \emph{recompile} the programs and \emph{reproduce} the vulnerabilities for their execution trace.
For all benchmarks, we first recompile these programs with {\tt gcov} flag --- a tool used in conjunction with GCC, to get the code coverage in programs.
Then we run the programs with the vulnerability inputs to get the \emph{code coverage report} and a typical code coverage report is shown in Figure~\ref{fig:report}. 
From the report, we can obtain the file name, the total and hit code lines and functions number, and the line coverage and function coverage of each program.
With the report, we can further extract the code execution traces of the vulnerabilities.
An example of the \emph{extracted execution trace} is shown in Figure~\ref{fig:code-coverage-example}.
% Then we rerun these buggy programs and obtain their code execution traces as Figure~\ref{fig:code-coverage-example}.
In the code execution trace, the lines of code which have been executed are marked pink, while the unexecuted lines are marked green.
For the 80 CVEs, we collect all the vulnerability reports for each CVE and \emph{set up the operating system and environment}.
After extracting the execution trace of a vulnerability, we manually analyze the \emph{path conditions} along the trace and the \emph{specific states} to fulfil for triggering the bug.

% In addition, we obtain unexpected behaviours (vulnerability types) from the bug reports. 

% \begin{figure}[t]
% \centering
%  \includegraphics[width=\linewidth]{figs/An-example-of-codecoverage-report}
% %\vspace{-0.2in}
% \caption{An example of code coverage report generated by {\tt gcov} in {\tt base64} of LAVA-M.}
% \label{fig:report}
% \end{figure}




% It should be noted that reproducing the vulnerabilities is extremely difficult and took us a lot of manpower.
% And we believe the 80 memory error vulnerabilities form a reasonably large dataset because recent work that uses vulnerabilities in the CVE list to evaluate their vulnerability detection systems are limited to less than 10 vulnerabilities~\cite{carlini2015control, hu2016data, castro2006securing, akritidis2008preventing}.




% It can be seen from the above that this is the largest analysis that manually verifies and confirms the differences between benchmarks and real-world vulnerabilities. 


\begin{figure}[b]
	\centering
	\includegraphics[width=0.35\textwidth]{figs/ccn_boxplot.pdf}
	\caption{Average Cyclomatic Complexity of Functions.}
	\label{fig:average-ccn-datasets}   
\end{figure}






\begin{figure*}[!htbp]
\centering
\begin{minipage}{0.47\linewidth}
 \includegraphics[width=\linewidth]{figs/An-example-of-codecoverage-report}
\vspace{-0.2in}
\caption{An example of code coverage report generated by {\tt gcov} in {\tt base64} of LAVA-M.}
\label{fig:report}
\vspace{-0.03in}
\end{minipage}
\hfill
\begin{minipage}{0.45\linewidth}
\includegraphics[width=\linewidth]{figs/An-example-of-codecoverage-in-base64-of-lava-m}
\vspace{-0.2in}
\caption{An example of program execution trace in {\tt base64} of LAVA-M.}
\label{fig:code-coverage-example}
\vspace{-0.03in}
\end{minipage}
\end{figure*}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figs/An-example-of-codecoverage-in-base64-of-lava-m}
% \caption{An example of program execution trace in {\tt base64} of LAVA-M.}
% \label{fig:code-coverage-example}
% \end{figure}









% On the whole, we collect two kinds of datasets, 
% one is a primary dataset identified by CVE IDs\cite{CVEWeb}, 
% the other is a supplementary dataset for vulnerabilities that
% do not have a CVE ID yet. At the same time, we also gather information from the National Vulnerability Database(NVD)\cite{NVDWeb}, a database with external references provided by the U.S.National Institute of Standards and Technology(NIST), which we can extract correlative information from. The relevant information includes the public disclosure dates, vulnerability classifications, the affected software repositories, most important of all, the proof-of-concept(PoC)files for each vulnerability. Figure describes the overview of this process. For the rest of this section, the various data sources of the real-world vulnerabilities and collection methodology will be described. 




==> prev/6-analysis-results.tex <==
\section{Analysis results}
\label{sec:analysis_results}


We will give our analytic results about the comparisons between artificial benchmarks and real-world ones, and answer to the three research questions.


\subsection{(Q1) How do the programs in artificial benchmarks differ from the programs containing real-world vulnerabilities?}
\label{sec:q1}


% \begin{table}[htbp]
% \scriptsize
% \centering

% \begin{tabular}{|p{1.6cm}|p{2.9cm}|p{2.9cm}|}
% \hline
% \textbf{Buggy program properties}     & \textbf{Discovery}                                                                                & \textbf{Rationale}                                                                                                           \\ \hline
% \textbf{Functionality diversity}      & LAVA-M and Rode0day are lack of functionality diversity, CGC is similar to the real world.          & Diversity help benchmarks better evaluate whether a bug finding tool is capable in various scenarios.                        \\ \hline
% \textbf{Lines of code (LOC)}          & The LOC of real-world programs are tens or hundreds of times more than that of benchmarks.        & The vulnerabilities in the small-sized benchmarks may be in a shallow depth and easier to be captured by a bug finding tool. \\ \hline
% \textbf{Cyclomatic complexity (CCN)} & Cyclomatic complexities of LAVA-M and Rode0day are similar to real world. CGC has lower complexity. & The simple logic inside the benchmarks can not evaluate the code coverage of bug finding tools.                              \\ \hline

% \end{tabular}
% \caption{Similarities and differences of buggy program properties between the programs in artificial benchmarks and the programs containing real-world vulnerabilities.}
% \label{tab:buggy program properties}
% \end{table}


% According to our model, the buggy programs come as the major component. 

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figs/An-example-of-codecoverage-in-base64-of-lava-m}
% \caption{An example of program execution trace in {\tt base64} of LAVA-M.}
% \label{fig:code-coverage-example}
% \end{figure}


In this section, to explore whether the buggy programs' inherent natures will influence the evaluation of the vulnerability detection tools, 
we will analyze the cyclomatic complexity of them.
Further, the feature affect the utility of some vulnerability
detection tools, especially the symbolic execution engine. Therefore, 
we additionally observe the performance of symbolic execution on
different benchmarks to support our analysis.


% We compare the similarities and differences between synthetic benchmarks and real-world programs as Table~\ref{tab:buggy program properties}.


\subsubsection{Cyclomatic complexity (CCN).}
% The program volume includes lines of code (LOC), cyclomatic complexity
% (CCN). Further, these features affect the utility of some vulnerability
% detection tools, especially the symbolic execution engine. Therefore, 
% we additionally observe the performance of symbolic execution on
% different benchmarks to support our analysis.

% \textbf{Lines of code (LOC) of the programs.}
% %We list the average LOC of three benchmarks and real-world programs in Figure~\ref{fig:average-LOC-datasets}. 
% Lines of code (LOC), is a software metric used to measure the size of a computer program by counting the number of lines in the text of the program's source code~\cite{Source_lines_of_code}.
% Based on our analytic results, the 40 real-world programs have an average of 178971 LOC, which is {\tt 58x} more than LAVA-M (3093), {\tt 14x} more than Rode0day (13037) and even {\tt 314x} more than CGC (570).

% The tremendous differences in LOC indicate a drawback in the scale of artificial programs. The vulnerabilities hidden in the small-sized benchmarks may be in a shallow depth and easier to be captured by a vulnerability detection tool compared with the real-world ones.

CCN is a quantitative measure of the number of linearly independent paths through a program's source code by using the control-flow graph of the program.
If the source code contained more control-flow statements (conditionals or decision points), the complexity would be more.
The higher the value of CCN is, the more complex the control flow of the program is~\cite{Cyclomatic_complexity}. 
We use a boxplot to show the average function level CCN for each dataset in Figure~\ref{fig:average-ccn-datasets}.
% A larger box means the average function level CCN values between different programs in the dataset are more discrete.
% A higher position of the box means a higher value of the average function level CCN.
% The bar inside the box shows the median value.
% We collect the median CCN in each dataset, listed in Table~\ref{tab:Cyclomatic-complexity-of-datasets}. 








We can clearly see that the average CCN values of Rode0day (9.1), LAVA-M (8.6), and real-world programs (8.1) are higher than the average CCN value of CGC (5.2).
The median CCN values of LAVA-M and Rode0day are similar to real-world ones because they exactly insert vulnerabilities to real-world programs.
% The results show that since LAVA and Rode0day insert bugs to programs of real world, their cyclomatic complexities are similar. 
% However, the programs in CGC have lower complexities, which indicates the logic inside these specialists' crafts is simpler than the real-world cases.
This indicates the logic inside these specialists' crafts (CGC) is simpler than the real-world cases.




% \textbf{Code coverage and function coverage of bug execution traces}.
% We studied the differences between the code coverages of the bug execution traces of the synthetic benchmarks and real-world programs.

% Based on the programs that recompiled with {\tt gcov} flag, we get the code execution trace, which represents the code lines that the programs execute along the trace. 
% We get the average code coverage and function coverage of datasets as Figure~\ref{fig:codelines&functions-coverage-of-datasets}. 

% For CGC, whose bugs are written by specialists, the code coverage and function coverage are nearly {\tt 3x} higher than the real-world programs and other benchmarks. 
% A higher coverage that the buggy input executes indicates it is easier for the symbolic executor to find the bugs~\cite{stephens2016driller}, which may be shallow or unrealistic. 
% So the code coverage of bugs execution test the scalability of the bug finding tool. 

% For LAVA-M and Rode0day, which automatically inject large numbers of bugs into programs, although their code coverage and function coverage are similar to that of the real world, the coverage of different bugs in one program is similar, even the same. 
% The coverage distribution is lack of diversity. 
% For example, in 49 bugs of {\tt grep} that inserted bugs by Rode0day, all of the code coverage and function coverage are 12.9\% and 18.6\%. 
% For 20 bugs of {\tt uniq} inserted by LAVA-M, half of the bugs' line coverage is 20.8\%, and the left is all 21.1\%.    

% \begin{figure}[htb]
% 	\centering
% 	\includegraphics[width=0.4\textwidth]{figs/codelines&functions-coverage-of-datasets.pdf}
% 	\caption{Code coverage and function coverage of datasets.}
% 	\label{fig:codelines&functions-coverage-of-datasets}   
% \end{figure}





\subsubsection{Effects to vulnerability detection tools.}

% \emph{\textbf{Effects to vulnerability detection tools.}}
How the features above affect the utility of some vulnerability detection tools?
To observe the performance of symbolic execution on different benchmarks, we evaluate how many vulnerabilities can be detected by the symbolic execution engine in LAVA-M and CGC. 
The reason why we only test with
symbolic execution is that the other prevalent category of 
vulnerability detection technique, fuzzing, has better scalability
and cannot well reveal the distinction in different datasets in terms of scalability.

The evaluation results are cited from LAVA~\cite{dolan2016lava}
and Driller~\cite{stephens2016driller}, and listed in
Table~\ref{tab:LAVA-M and CGC detected by SE}.
As the result shows, the vulnerabilities of LAVA-M detected by symbolic 
execution only account for 1.2\% of the 2265 total vulnerabilities, 
but CGC is {\tt 12x} more than LAVA-M and the percentage is 12.7\%.
We ascribe the easier detection by symbolic execution in CGC
to its much simpler program logic. Thus, we
conclude that, as a benchmark, the complexity of control-flow  of CGC is too simple to evaluate if the tools can detect vulnerabilities of larger programs so it can not evaluate the scalability 
of vulnerability detection tools well, especially symbolic execution technique.


\begin{table}[htbp]
\centering
\caption{The number of vulnerabilities that detected by symbolic execution in LAVA-M and CGC.}
\label{tab:LAVA-M and CGC detected by SE}
\begin{tabular}{c|c|c|c}
\toprule[1.3pt]
\textbf{Dataset} & \textbf{Detected} & \textbf{Total} & \textbf{Percentage} \\ \hline
\textbf{LAVA-M}  & 27                & 2265           & 1.2\%              \\ \hline
\textbf{CGC}     & 16                & 126            & 12.7\%             \\ 
\bottomrule[1.3pt]
\end{tabular}


\end{table}


The cyclomatic complexity of artificial benchmarks can influence the evaluation of vulnerability detection tools whether they can detect more complicated programs and will affect the evaluation on the \emph{scalability} of tools.
From our analysis, the cyclomatic complexity varies in some degree between the programs of artificial benchmarks and real world containing vulnerabilities, so they \emph{insufficiently} represent the reality in this aspect.






% \subsubsection{Functionality diversity}
% Functionality diversity refers to whether the functions of programs are diverse or not.
% Though LAVA-M injects 587 bugs into four programs, they are all inserted in GNU Core Utilities and \emph{realize one functionality}. 
% Similarly, Rode0day injects 1963 bugs into nine programs, but only \emph{accomplish five functionalities} (eg. file compression programs, database management system and JavaScript engine).
% For CGC, programs are written by specialists and \emph{realize dozens of functionalities}, such as an electronic calculator, a multi-player game, even a chat room, etc.
% For real-world programs, our dataset of 80 real-world programs includes \emph{{\tt 40} different functions}, like converter, XML Parser, servers, etc, which are far richer than {\tt 1} in LAVA-M and {\tt 5} in Rode0day. 

% From the statistics, we can observe that the programs chosen by LAVA-M and Rode0day are \emph{lack of functionality diversity}. 
% CGC is \emph{similar} to the real-world programs with a variety of functionalities. This diversity will help the benchmarks better evaluate the \emph{generality} of vulnerability detection tools, typically whether they are capable of various scenarios.


\begin{tcolorbox}[size=title, opacityfill=0.15]
Though some of the program properties share similarities, there still exist significant differences between artificial benchmarks and reality, which may lead to the distinctions to the depth and difficulty for both bug insertion and discovery.
Furthermore, they can influence the scalability of the vulnerability detection tools.
\end{tcolorbox}



\subsection{(Q2) How do artificial vulnerabilities differ from real-world vulnerabilities? Can artificial vulnerabilities sufficiently mirror the reality?}
\label{sec:q2}

% \begin{table}[htbp]
% \scriptsize
% \centering
% \begin{tabular}{|p{1.6cm}|p{3cm}|p{3cm}|}
% \hline
% \textbf{Bugs properties} & \textbf{Discovery} & \textbf{Rationale}\\ \hline
% \textbf{Requirements to trigger the bug.} & 
% % [c]{@{}l@{}}
% % \begin{tabular}{p{2.8cm}}
% \textbf{Reach the buggy location.} Distribution, types of magic numbers and data flow in LAVA-M and Rode0day are far away from the real-world vulnerabilities, CGC designed by specialists can be more freely and seem more realistic.

% \textbf{Trigger specific states.} Bugs inserted by LAVA-M and Rode0day can cause a crash without triggering specific states and different from bugs of real world and CGC programs.
% % \end{tabular} 

% & Buggy location and specific states evaluate the ability of solving constraints and code coverage of the bug finding tools. \\ \hline

% \textbf{Bug/unexpected behavior types.}                                         & LAVA-M and Rode0day only can insert single bug type. Though CGC can insert many types of bugs, they are not exactly the same as the real-world ones.                                                                                                                                                                                                                                                                                                        & Different types of bugs require different approaches to test the versatility of the bug finding tool.                      \\ \hline
% \textbf{Code coverage and function coverage of the execution trace of the bug.} & The coverage distribution of LAVA-M and Rode0day is lack of diversity. CGC is 3x lower than the real-world programs.                                                                                                                                                                                                                                                                                                                          & Code coverage of bugs execution test the scalability of the bug finding tool.                                              \\ \hline
% \end{tabular}
% \caption{Bug properties of artificial vulnerabilities and real-world vulnerabilities.}
% \label{tab:buggy properties}
% \end{table}



From the above analysis, we observe the program properties of artificial benchmarks and real world are different in some aspects.
In this section, we further explore the differences between artificial vulnerabilities and real-world ones.

We first analyze the properties of vulnerabilities in the dataset.
We depict the differences from two aspects:
the \textbf{requirements to trigger the vulnerability} and 
the \textbf{unexpected behaviour types} as the model. 
% Besides these two aspects, we also analyzed code coverage and function coverage of the execution trace of the bug to further study about the differences between the synthetic benchmarks and real-world programs as Tabel~\ref{tab:buggy properties}. 
Then we modify the artificial benchmarks in accordance with
the features we summarized for the real-world vulnerabilities, 
and test them with the vulnerability detection tool AFL~\cite{AFL}.
The detected vulnerability number dissimilarity well represents the benchmarks can \emph{not} mirror the reality.

% For the comparison between benchmarks and real-world vulnerabilities, we analyze from five aspects based on the model, which are the bug types, requirements to trigger a vulnerability, the difficulty of reaching different path conditions and the types of magic number, characteristics of data flow and code coverage and function coverage. 




\subsubsection{Requirements to trigger a vulnerability.}
As our model mentioned, a crash needs two requirements which are reaching the buggy location and triggering specific states along the execution trace.

\ding{182} We analyze the differences in \emph{reaching the buggy location} from the perspectives of control flow and data flow.

First, for the perspective of \emph{control flow}, we will give the comparisons from three aspects.
Before reaching the buggy location, the program execution
must meet a certain number of path conditions. 
However, some of the paths are protected by magic bytes comparisons, and can only be reached when the detection tools solve
the corresponding constraints. 


\textbf{The types and proportions of magic numbers.}
We summarize the types of magic numbers and their
proportions in Table~\ref{tab:Magic-number-type-of-datasets}.
The comparisons in LAVA-M and Rode0day cover only two types
and are almost 32-bit. In contrast, CGC and 
real-world programs have various types of magic numbers.
When we further
study the proportion of each type, we find that
though LAVA-M and Rode0Day put nearly 90\% of their efforts on
the type of {\tt int32}, it only accounts for 17\% in the 
real world. In addition, all benchmarks do not compare the type 
of {\tt unsigned int 16}, {\tt32} and {\tt long int}.

To summarize, since the distribution and the types of 
magic numbers in LAVA-M and Rode0day are far away from the
real-world vulnerabilities, they may not 
evaluate the ability to solve constraints of 
the vulnerability detection tools as fairly as the real world.
As CGC is written by specialists, their magic numbers can
be designed more freely and seem more realistic.

\begin{table}[h]
\centering
\caption{Magic number type of datasets.}
\label{tab:Magic-number-type-of-datasets}
\begin{tabular}{c|c|c|c|c}
\bottomrule[1.3pt]
\textbf{\begin{tabular}[c]{@{}c@{}}Magic Number \\ Type\end{tabular}} & \textbf{LAVA-M} & \textbf{Rode0day} & \textbf{CGC} & \textbf{Real World} \\ \hline
\textbf{char}                                                         & 8\%             & 10\%              & 40\%         & 51\%                \\ \hline
\textbf{string}                                                       & -                & 3\%               & 29\%         & 26\%                \\ \hline
\textbf{float}                                                        & -                & -                  & 5\%          & -                    \\ \hline
\textbf{unsigned int16}                                               & -                & -                  & 0.5\%        & 1\%                 \\ \hline
\textbf{unsigned int32}                                               & -                & -                  & 3\%          & 4\%                 \\ \hline
\textbf{unsigned int64}                                               & -                & -                  & 0.5\%        & -                    \\ \hline
\textbf{int32}                                                        & 92\%              & 87\%              & 21.5\%       & 17\%                \\ \hline
\textbf{long int}                                                     & -                & -                  & 0.5\%        & 1\%                 \\ 
\bottomrule[1.3pt]
\end{tabular}


\end{table}

\textbf{Difficulty of solving the constraints.}
For LAVA-M and Rode0day, we observe there are few or simple 
comparisons against magic numbers along the trace. 
But at the position where they insert bugs, the comparisons
are against 32-bit magic constants, which are unusually
difficult to find by fuzzing tools like AFL~\cite{AFL}. 
In a word, the difficulty of solving the magic 
numbers becomes harder noticeably in the last if-condition. 
However, in CGC and the real-world CVEs, we
observe that such difficulty is in an even distribution.




% \textbf{The lines coverage and functions coverage of execution traces of bugs.}
% The code coverage is an important metric to observe the depth and breadth of an execution trace. 
% We obtain the lines and functions coverage of all the execution traces of artificial and real-world vulnerabilities.
% %, and randomly select some files as examples. 
% Figure~\ref{fig:Lines-Coverage} and Figure~\ref{fig:Function-Coverage} show the results.
% Since we have too many programs and put them all in one figure is overwhelming, the two figures only show the sample programs we randomly selected from each dataset.
% For LAVA-M or Rode0day, we can clearly see from both figures that the execution trace coverages for different vulnerabilities do not differ very much.
% This means LAVA-M or Rode0day inject bugs into similar locations.


% In programs which are inserted with several bugs by LAVA-M or Rode0day, we observe each line coverage and function coverage has a high similarity, especially, in the same program looks like a straight line in the figures.
% Also, the lines and functions coverage are similar among multiple programs respectively.



% On the contrary, the lines coverage and functions coverage of the execution traces of CGC vulnerabilities are sparse, ranging from 4.2\% to 100\%. 
% This is similar to the real-world situation, where vulnerabilities sparsely disperse in the programs.
% Moreover, sparsely distributed vulnerabilities require the testing tool to cover more program states.
% To sum up, we can see that LAVA-M and Rode0day do not evaluate the \emph{program state coverage} capability of the vulnerability detection tools well, while CGC is better in this aspect.


% And the real-world vulnerabilities are also dispersive among various programs.
% If the line coverage is diversity, it can better evaluate whether the vulnerability detection tools can cover more program state coverage and solve out the constraints.
% So the bugs inserted by LAVA-M and Rode0day are similar and can not evaluate the \emph{program state coverage} of vulnerability detection tools well, while CGC is better for this aspect. 
% The analysis results show that LAVA-M and Rode0day are not 

% \begin{figure}[!ht]
% 	\centering
% 	\includegraphics[width=0.35\textwidth]{figs/Lines-Coverage.pdf}
% 	\caption{Lines coverage of the programs of datasets.}
% 	\label{fig:Lines-Coverage}   
% \end{figure}

% \begin{figure}[!ht]
% 	\centering
% 	\includegraphics[width=0.35\textwidth]{figs/Function-Coverage.pdf}
% 	\caption{Functions coverage of the programs of datasets.}
% 	\label{fig:Function-Coverage}   
% \end{figure}

% \begin{figure*}[!ht]
% \centering
% \begin{minipage}{0.35\linewidth}
% \includegraphics[width=\linewidth]{figs/Lines-Coverage.pdf}
% \vspace{-0.2in}
% \caption{Lines Coverage of the programs of datasets.}
% \label{fig:Lines-Coverage}
% \vspace{-0.03in}
% \end{minipage}
% \hfill
% \centering
% \begin{minipage}{0.35\linewidth}
% \includegraphics[width=\linewidth]{figs/Function-Coverage.pdf}
% \vspace{-0.2in}
% \caption{Functions Coverage of the programs of datasets.}
% \label{fig:Function-Coverage}
% \vspace{-0.03in}
% \end{minipage}
% \end{figure*}


Second, as to the perspective of \emph{data flow},
we will give the comparisons from three aspects.

\textbf{The data used to insert bugs.} 
In order to insert bugs to the programs, as mentioned in Section~\ref{section:Background}, LAVA-M and Rode0day use DUAs and subvert them to introduce memory corruption errors into the program’s source.
Since such DUAs is \emph{unused} because its value is never read before the next time it is written, which means LAVA can safely overwrite the variable with the designed data without affecting the the program's execution because no subsequent portion of the program relies on or is affected by the variable's current value. 
However, the vulnerabilities in the real world are oftentimes triggered by some useful input data other than the unused DUAs.


\textbf{The proportion of data transformation in the trace.}
At the points where LAVA-M and Rode0day insert bugs, the values of magic numbers are often the direct copies of inputs without any data transformation. 
Our statistics of the real world and CGC in Table~\ref{tab:data-transformation-of-datasets} show that 61.8\% of inputs in real-world programs have data transformations, including but not limited to type conversion, casting the integer to the character or doing inversely and bit-wise operation in real-world. 
As to CGC, only 40\% of them have data transformations along the trace, where type conversion is the majority.   


\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{5mm}{
\caption{The proportion of data transformation of datasets.}
\label{tab:data-transformation-of-datasets}
\begin{tabular}{c|c|c}
\toprule[1.3pt]
\multicolumn{1}{c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{Transformation}} & \multicolumn{1}{c}{\textbf{Non-Transformation}} \\ \hline
LAVA-M                                  & 0\%                                          & 100\%                                           \\ \hline
Rode0day                              & 8\%                                          & 92\%                                           \\ \hline
CGC                                   & 40.0\%                                       & 60.0\%                                          \\ \hline
Real World                            & 61.8\%                                       & 38.2\%                                          \\ 
\bottomrule[1.3pt]
\end{tabular}}


\end{table}


\textbf{The property of the data flow.} 
The data flow created by LAVA-M or Rode0day is artificial because the DUA and the attack point (ATP) are independently chosen out of a set of candidate DUAs and candidate ATPs.
So the two points in the program are not likely to have any semantic relationship with each other. 
The {\tt lava\_get()} and {\tt lava\_set()} methods will then introduce an arbitrary connection. 
But the data flow of real-world programs is realistic and has a semantic association with each other. 
Rode0day adds data flow between DUAs and ATPs by adding an additional argument {\tt int* lava} to each of the shaded functions. 
But the approach also brings with limitations. Rode0day can not modify library functions and when control flow passes to a library function, all the call functions after that are inaccessible for data flow and bug insertion. 




In summary, the data flow created by LAVA-M and Rode0day is artificial and unrealistic, and there is no data transformation along the trace. Although CGC makes some data transformation, there still exists a gap between the real world and CGC.


\ding{183} The differences in the perspective of triggering specific program states.

\textbf{Triggering specific program state conditions.}
As have mentioned before, since LAVA-M and Rode0day artificially construct the relation between DUA and ATP, the execution trace to trigger the vulnerability must fulfill the series of path conditions designated by them, including the magic number guarded at the last path comparison.
As to LAVA-M, once the magic number of the last if-condition is solved out, the program will crash immediately without any specific state to be triggered along the trace.
Though Rode0day has improved LAVA by using multiple DUAs in the last conditions to complicate the comparisons, its vulnerability triggering mechanism still excludes any specific state.

The vulnerabilities in the real world and CGC reveal the opposite feature at the time of crash.
To make a memory corruption vulnerability, it must go through some specific states and trigger that.
For example, as for Buffer-Overflow vulnerability, the program should read or write a longer size of data to the buffer allocated, that is, if it triggers the specific states, the program will crash successfully.
As for use-after-free vulnerability, before the pointer used, it must be freed first, which triggers a specific state.

\begin{figure}[!ht]
\begin{lstlisting}[language=c,
xleftmargin=.05\columnwidth, xrightmargin=.01\columnwidth,
% xleftmargin=.08\columnwidth, xrightmargin=.03\columnwidth,
% linewidth=.95\columnwidth, 
linebackgroundcolor={%
\ifnum\value{lstnumber}>4\ifnum\value{lstnumber}<6\mtcolor\fi\fi
\ifnum\value{lstnumber}>11\ifnum\value{lstnumber}<14\mtcolor\fi\fi
}]
void receive_input(FILE *f){
    ...
    char buf[1024];
    fread(buf, 1024, 1, f);
    lava_set(*(int *)buf);
    ...
}
...
void foo(char *bar){
    // BUG:

    printf("%s\n", bar + lava_get() * 
    (lava_get() == 0x6176616c));
}
\end{lstlisting}
\caption{A bug inserted by LAVA-M.}
\label{lis:lava-bug}
\end{figure}


\begin{figure}[ht]
\begin{lstlisting}[language=c,
xleftmargin=.05\columnwidth, xrightmargin=.01\columnwidth,
% xleftmargin=.08\columnwidth, xrightmargin=.03\columnwidth,
% linewidth=.95\columnwidth, 
linebackgroundcolor={%
\ifnum\value{lstnumber}>4\ifnum\value{lstnumber}<6\mtcolor\fi\fi
\ifnum\value{lstnumber}>8\ifnum\value{lstnumber}<10\mtcolor\fi\fi
}]
void ReadFace(fbuf){
    ...
    t = s = fbuf;
    if(...){
        char buffer[128];
        sscanf(s, "%s %s", buffer);}
        ...
    c = (int)* (s++);
    if((c >= '0') && (c <= '9'))
    ...
\end{lstlisting}
\caption{A buffer overflow vulnerability in CVE-2009-2286.}
\label{lis:cve-bug}
\end{figure}


In the following, we present a detailed \textit{case study} to illustrate the difference in triggering specific states between benchmarks and real-world vulnerabilities.

Figure~\ref{lis:lava-bug} shows an example bug inserted by LAVA-M.
The function {\tt lava\_get} retrieves the value last stored by a call to {\tt lava\_set}.
Once the magic number {\tt 0x6176616c} is solved out, the program will crash even without any specific state to be triggered.


On the contrary of real world, taking CVE-2009-2286 in Figure~\ref{lis:cve-bug} as an example, we can observe that
when the input solely reaches the last condition 
{\tt if((c>='0')\&\&(c<='9'))},
the buffer overflow vulnerability in {\tt ReadFace} may \emph{not} be triggered. 
Unless the size of input is longer than 128 that the buffer allocated, the program will only crash successfully.


To sum up, for the bugs artificially inserted by LAVA-M and Rode0day,
their triggering conditions are deliberately designed 
but distinct from the true circumstances under the real world. 
Such design may not well evaluate the ability of 
\emph{program state coverage} exploration for vulnerability detection tools.



\subsubsection{Unexpected behaviour types} 
Unexpected behaviour types, also called vulnerability type, can evaluate the sensitivity of vulnerability detection tools.
If the tools are less effective, they can not detect diverse vulnerability types.

LAVA and Rode0day can inject \emph{only} buffer overflow bugs into programs, and CGC has many different types of bugs, including but not limited to Buffer-Overflow, Null-Pointer-Dereference, Use-After-Free.
As for the vulnerabilities of real world, we look up to the 5 most common memory corruption vulnerabilities in real world~\cite{CWEWeb}. 
We count about 93 challenges with 119 bugs of CGC accordingly as Table~\ref{tab:CGC-Realworld-Bug-Type}. 
Noted that because one challenge may include more than one bug, the total numbers of CGC's bugs (in the last column of Table~\ref{tab:CGC-Realworld-Bug-Type}) are larger than the number of CGC's challenges we collected.

The results show that the top 3 bugs type of CGC are Out-of-Bounds Write, Out-of-Bounds Read, and Null-Pointer-Dereference, which account for 37.8\%, 22.7\% and 20.2\% of the total bugs we collected respectively. 
Compared to the real world, however, the same bug types only account for 3.4\%, 8.6\% and 5.0\% respectively, which indicates the great difference of the bug type distribution between CGC and real world. 

As the result shows that the bugs that LAVA-M and Rode0day can insert are in a single form. 
Though CGC has many types of bugs, the percents are much less than the real-world circumstances.
A probable reason why CGC has more Out-of-Bounds Writing and Reading bugs is that they are easier to create.
The benchmarks that lack diversity in inserted bugs may not well
evaluate the \emph{sensitivity} of vulnerability detection tools, since certain
bugs excluded from the benchmarks may not be detected by some
less effective tools.




\begin{table}[hbp]
\scriptsize
\centering
\caption{The 5 most common software weaknesses of memory corruption vulnerabilities in real world~\cite{CWEWeb}, and the number of them in CGC.}
\label{tab:CGC-Realworld-Bug-Type}
\begin{tabular}{c|c|c|c}
\toprule[1.3pt]
   & \textbf{\begin{tabular}[c]{@{}c@{}}Weakness \\ Summary\end{tabular}}                                          & \textbf{\begin{tabular}[c]{@{}c@{}}Real-World \\ Num  (Percentage)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}CGC \\ Num  (Percentage)\end{tabular}} \\ \hline
1              & Buffer-Overflow          & 12293 (76.3\%)                                                                      & 14 (11.7\%)                                                                  \\ \hline
2              & Out-of-Bounds Read                                                 & 1390 (8.6\%)                                                                        & 27 (22.7\%)                                                                  \\ \hline
3              & Use-After-Free                                                     & 1079 (6.7\%)                                                                        & 9 (7.6\%)                                                                    \\ \hline
4              & \begin{tabular}[c]{@{}c@{}}Null-Pointer\\ -Dereference\end{tabular} & 805 (5.0\%)                                                                         & 24 (20.2\%)                                                                  \\ \hline
5              & Out-of-Bounds Write                                                & 548 (3.4\%)                                                                         & 45 (37.8\%)                                                                  \\ 
\bottomrule[1.3pt]
\end{tabular}
\end{table}


\subsubsection{Benchmark modification}
The above analytic results all indicate that the vulnerability
features in the artificial benchmarks differ greatly from
the real world. Thus, we further carry on a series of experiments 
to evaluate how these differences will affect the utilities of
vulnerability detection tools. 
Our experiments are only conducted on LAVA-M because
Rode0day is evolved from LAVA with a similarly unsatisfactory
manifestation in our model, 
while CGC is written by specialists and its features are close
to the reality in most metrics.

% We first modify the benchmark vulnerabilities to be more
% realistic and eliminate such differences as much as possible.
% Based on the programs which have already been inserted vulnerabilities
% in LAVA-M, we make modifications from the following four aspects.
First, we modify the program in LAVA-M to make it more realistic from the following aspects:
\ding{182}We extend the magic number types to {\tt char}, {\tt string} and {\tt int32} (we omit the types that account for less 
than 5\% in Table~\ref{tab:Magic-number-type-of-datasets}) by modifying \emph{if conditions}, with a similar proportion to real-world cases.
\ding{183}We add extra \emph{data transformation} to the DUAs before they are compared to the magic number.
\ding{184}We combine \emph{both} the above modifications.
% \begin{itemize}
% \item We extend the magic number types to {\tt char}, {\tt string}
% and {\tt int32} (we omit the types that account for less 
% than 5\% in Table~\ref{tab:Magic-number-type-of-datasets}), with a similar proportion to real-world cases.
% \item We add extra data transformation to the DUAs before they are compared to the magic number.
% \item We combine both the above modifications and apply to base64.
% %\item We add data transformation to the DUAs before they are compared to the magic number.
% %\item We change the Buffer-Overflow vulnerabilities to Double-Free.\yunlan{Need to explain why we change them to Double-Free in the following result analysis.(Some bug finding tools cannot detect such vulnerabilities that do not lead to the crash.)}
% %\item We combine the modification to data transformation and magic number types.
% \end{itemize}
% By applying the aforementioned modifications
% , we obtain 3 different versions of base64:
% the one with \textit{if conditions} modified;
% the one with \textit{data transformations} added;
% the one with both modified \textit{if} conditions and added \textit{data transformations}.
% Finally we utilize AFL to detect the bugs and see how the changes influence the properties of vulnerability detection tool.
Considering the high similarity between the LAVA-inserted bugs in 
different programs, we only modify {\tt base64} in LAVA-M.
After applying these modifications, we obtain 3 different versions 
of {\tt base64}, and run AFL on them respectively, as well as the 
original {\tt base64} in LAVA-M.
Each of the experiments is repeated 5 times to mitigate the randomness of fuzzing and lasts for 5 hours to align with~\cite{dolan2016lava,li2017steelix,rawat2017vuzzer}.
%\footnote{We repeat the experiments to mitigate the randomness of fuzzing; we use 5-hour here to align with~\cite{dolan2016lava,li2017steelix,rawat2017vuzzer}.}
Lastly, we collect the unique crashes detected by AFL in the experiments to evaluate the effects of the modifications.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.35\textwidth]{figs/base64_overall-crash-time.pdf}
	\caption{Crashes detected by AFL in 5 hours. The shaded area is the 95\% confidence interval. ``if" means the if conditions are modified; ``dt" means data transformation is added; ``if-dt" means both are modified; ``orig" means original {\tt base64}.}
	\label{fig:crashes_base64}   
\end{figure}
%\vspace{-6pt}

Figure~\ref{fig:crashes_base64} shows the average number of unique crashes detected by AFL during the experiments.
We can see that modifying the \textit{if conditions} makes it much easier for AFL to detect the bugs.
This is because almost half of the comparisons in real-world cases are \texttt{char} comparisons, which are easier for AFL to penetrate.
Adding \textit{data transformations} makes it harder for AFL to detect bugs. 
In fact, AFL detects no bug in this version of {\tt base64}.
However, the difference between this version and the original version is minor as the 95\% confidence intervals overlap and the p-value of Mann-Whitney U test is 0.212, above 0.05.
Because the bugs are already hard for AFL to detect, making it harder does not cause big differences.
The version applying both \textit{if conditions} modification and \textit{data transformation} addition is closest to real-world cases.
The number of unique crashes detected is between the other 2 modified versions as expected.
However, the results on this realistic version differ very much from the results on the original version as the confidences intervals are discrete and the p-value is 0.005, below 0.05.
The results of the experiments show that the artificial bugs cannot mirror the reality well because they may not fairly reflect the properties of the vulnerability detection tool.





% The results shows as follows.
% \scarlett{explain the results.}
% We can see that the realistic changes as real world to the programs of LAVA-M varies differently from LAVA-M.
% And LAVA-M can not sufficiently mirror the reality in some degree.
% They can not evaluate vulnerability finding tools well in program state coverage and sensitivity.


















\begin{tcolorbox}[size=title, opacityfill=0.15]
Through the above analysis, we can see the benchmarks and the real-world vulnerabilities have different manifestations on our model and can not evaluate vulnerability detection tools well in the aspects of program state coverage and sensitivity. 
\end{tcolorbox}



\subsection{(Q3) What improvements can we make towards more realistic artificial vulnerabilities benchmarks?}
\label{sec:q3}

% To improve the quality of benchmarks, it is likely that some effort is needed from previous work. 
% Here, we discuss the possible approaches from the perspectives of data flow and control flow to make the benchmark closer to real-world bugs.

In this section, we discuss how to make the artificial benchmark more realistic based on two aspects of the program (corresponding to \textbf{Q1}) and vulnerability (corresponding to \textbf{Q2}).

\textbf{From the program perspective,} we can:
\ding{182} make the benchmark programs \emph{diverse in functionality}.
The benchmark should include programs with various functionalities to cover different scenarios and test the generality of the vulnerability detection techniques.
\ding{183} make the \emph{LOC and complexity of the programs similar to real-world programs}.
This means the volume of the benchmark programs should not be too small to test the scalability of the vulnerability detection technique.

\textbf{From the vulnerability perspective,} we can:
\ding{182} \emph{uniformly distribute} the path conditions base on their difficulties.
This is because we find that the difficulties of path conditions are biased.
Adding a hard-to-match magic number by the end of the path can make it harder to vulnerability techniques for detection but cannot represent the path conditions in real-world programs.
\ding{183} \emph{add some data transformations} along the execution trace of vulnerabilities.
We found that the input data goes through data transformations on real-world vulnerabilities.
Moreover, adding data transformations is in fact how Rode0day is evolved from LAVA.
This is complementary to distributing the path conditions, which also helps to test out the program coverage capability of vulnerability detection tools.
\ding{184} \emph{set proper special states} as requirements for triggering the artificial vulnerabilities.
We found that only reaching the buggy location is often not enough to trigger the vulnerabilities in real-world cases.
An artificial vulnerability should have a certain program state as its prerequisite to better represent the real-world case.
This can help to test out the program state exploration capability of the vulnerability detection tools and is complementary to the two previous suggestions which are related to making the buggy location hard to reach.
\ding{185} \emph{add different types of vulnerabilities}.
Different types of vulnerabilities often require different approaches for effective detection.
This can help to test the versatility and sensitivity of the detection tool.


% \textbf{Make the functionality of the programs diverse.}
% The programs that inserted bugs should be diverse, and the functionalities should be various rather than single. 
% 
% \textbf{Lines of code (LOC) should be similar to the real world .}
% The lines of code should not too small like CGC programs, it should include more lines to be realistic.
% 
% \textbf{Increase the cyclomatic complexity of programs.}
% Make the logic of programs more complex as the programs of real-world, and have a realistic control flow.

% \textbf{Add multiple bug types.}
% Broaden the diversity of types of bugs and do not just buffer overflow types as LAVA and Rode0day.
% There can be use-after-free, null-pointer-dereference and so on.
% 
% \textbf{Add data transformations along the trace.} 
% When artificial bugs are inserted to programs, we need to keep the diversity of data transformations along the executing trace from start to end as the bugs of real-world programs so that the input is not compared directly with magic numbers. 
% For example, there can be type conversion, such as casting the integer to the character or doing inversely. 
% Also, there can be bit-wise operation and encoding. 
% Besides this, the transformation between unsigned and signed is alternative. 
% 
% \textbf{Set a proper or specific state to be triggered for the crash.}
% Instead of the original rigid implantation, such as merely resolving magic number as LAVA and Rode0day, we need to let the programs meet some specific states, such as reading or writing a longer size of data to the buffer allocated for buffer overflow vulnerabilities. 
% 
% 
% \textbf{Make a uniform difficulty of reaching path conditions.}
% The difficulty to solve the magic bytes should be in an even distribution but not harder noticeably. 
% For example, the magic number can be one-byte and two-byte in the next condition, but not change to 4-byte immediately.  


\begin{tcolorbox}[size=title, opacityfill=0.15]
With the model and the analysis of different artificial benchmarks as well as programs, we provide suggestions from the program and vulnerability perspectives for building a more realistic benchmark.
% And we give some suggestions based on our model and make the bugs more realistic as real world instead of the original rigid implantation, which is a better direction for the development of the benchmarks.
\end{tcolorbox}


 











==> prev/7-related-work.tex <==
\section{Related work}
\label{sec:related}
% There is a body of work comparing benchmarks that used widely and real-world vulnerabilities in multi-dimension. 
% In the following, we summarize the key existing relevant works and highlight the uniqueness of our work. 
% For the existing works, We focus our discussion on introducing the benchmarks, evaluation of bug finding tools with benchmark and study on the vulnerabilities of real world.
Since this work is the first one to systematically study the artificial
and real-world vulnerabilities and explain how benchmarks evaluate 
the vulnerability detection tools, we focus on the related work from three categories: the artificial benchmarks, studies about real-world vulnerabilities and the vulnerability detection tools.

% \subsection{Benchmark}
\textbf{Artificial Benchmarks.}
There are some artificial benchmarks to evaluate vulnerability detection tools~\cite{dolan2016lava, pewny2016evilcoder, Rode0dayWeb, CGCWeb, hu2018chaff, roy2018bug}.
Most of the works automatically inject bugs to benign programs while in CGC every program is written by experts manually with purposely introduced bugs.
Besides the three most-used benchmarks we study,
% LAVA-M~\cite{dolan2016lava}, Rode0day~\cite{Rode0dayWeb} and CGC~\cite{CGCWeb} are the artificial benchmarks studied in this work and detailed in Section~\ref{sec:dataset_bg}.
% LAVA~\cite{dolan2016lava} add a sufficient number of new bugs for purposes of testing bug finding tools. 
% DARPA Cyber Grand Challenge (CGC), a competition designed to “test the abilities of a new generation of fully automated cyber defense systems”~\cite{CGCWeb}. 
% Rode0day~\cite{Rode0dayWeb}, a recurring bug finding competition and uses automated bug insertion techniques to which a tool could overfit.
Evilcoder~\cite{pewny2016evilcoder} automatically find potentially vulnerable source code locations and transform benign code into vulnerable code.  
% Chaff Bugs~\cite{hu2018chaff} add large numbers of bugs that are provably (but not obviously) non-exploitable to make attackers who attempt to find and exploit bugs in software will with high probability and waste precious resources in trying to build a working exploit. 
Bug Synthesis~\cite{roy2018bug} uses symbolic execution and constraint-based program synthesis to automatically inject bugs.
%Instead of studying every artificial benchmark, we analyzed the three most representative datasets and proposed strategies for improving these benchmarks. 
Unlike the above works which focus on building new benchmarks,
we concentrate on systematically studying the differences between the three most-used artificial benchmarks and real-world vulnerabilities. 



%\subsection{Study on the vulnerabilities of real-world}
\textbf{Studies of Real-world Vulnerabilities}
% In the field of software security, memory corruption bugs in software written in low-level languages like C or C++ are one of the oldest problems~\cite{szekeres2013sok}. 
% As memory corruption vulnerabilities, like use-after-free~\cite{caballero2012undangle, lee2015preventing, younan2015freesentry, van2017dangsan}，null-pointer-deference\cite{farzan2012predicting, ma2008computing} and so on.     
Several works have been proposed to study the properties of real-world vulnerabilities~\cite{walden2014, fabian2014, leopard2018}.
Their main purposes are different from ours.
They focus on detecting real-world vulnerabilities with the metrics while we focus on comparing real-world vulnerabilities with artificial bugs.

% Unlike previous works that mainly focus on implementing new benchmarks, they do not analysis detailed why the previous used widely benchmarks are not as realistic as the bugs of real-world programs, or only mentioned once.

% Our work first extracts the conditions for triggering a memory corruption vulnerability, then propose a model including program properties and vulnerability conditions. 
% Based on our model, we conduct an in-depth empirical analysis with multi-dimension on the benchmarks and bugs of real world. 
% Follow three research questions, we show that the bugs inserted to programs artificially is unrealistic in some way and it can not represent the bugs of real-world programs. 
% 
% To the best of our knowledge, this is the first study to provide an in-depth analysis of the comparison between benchmarks and bugs of real world. 
% Additionally, this is the first work to study a large number of bugs inserted into programs artificially and real-world vulnerabilities through extensive manual efforts.




%\subsection{Bug finding tools evaluation with benchmarks}
%\textbf{Bug finding tools evaluation with benchmarks}
\textbf{Vulnerability Detection Tools.}
The major purpose of benchmarks is to evaluate vulnerability detection tools.
% The ultimate measure of a bug finding tool is the number of distinct bugs that it finds.
% A better approach is to measure against ground truth directly by assessing fuzzers using a synthetic suite such as CGC or LAVA. 
Rise of the HaCRS~\cite{shoshitaishvili2017rise} and  Driller~\cite{stephens2016driller} use CGC as the benchmark. 
VUzzer~\cite{rawat2017vuzzer}, Steelix~\cite{li2017steelix} and QSYM~\cite{yun2018qsym} use LAVA-M as the ground-truth. 
But few published vulnerability detection tools use Rode0day for evaluation because it is a very recent work. 
The aforementioned tools also use real-world programs as ground truth, like {\tt nm}, {\tt objdump} and {\tt gif2png}, etc.
%In this work, we evaluate the most widely-used artificial benchmarks and programs adopted by these tools.
% For example, {\tt FFmpeg-n0.5.10} was used in FuzzSim~\cite{woo2013scheduling}, {\tt binutils-2.26} was the subject of the AFLFast evaluation~\cite{bohme2017coverage}, {\tt gif2png-2.5.8} was tested by VUzzer.

==> prev/8-future-work.tex <==
\section{Future Work}

Our future work primarily focuses on implementing a new benchmark. 
For example, our findings suggest that adding data transformations along the trace and making a uniform difficulty for reaching path conditions are more realistic for creating bugs artificially. 
Instead of the original rigid implantation, the bugs inserted to the programs need realistic data flow and control flow. 
Broadening the diversity of types of bugs and injecting exploitable bugs explicitly are also future directions for our work. 

Moreover, we will explore the current state of vulnerability discovery and software security based on our analysis results, like what properties make a given bug difficult to find and what types of bugs are currently missed by existing vulnerability finding tools. 
This can inform us of how to improve the state-of-the-art in the field of vulnerability discovery.  

==> prev/9-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This work presents an in-depth empirical study on artificial vulnerability 
benchmarks, with the goal of understanding how close these
benchmarks represent the reality. To maintain the generality and 
objectiveness, our study covers three most-used artificial 
benchmarks of 2669 bugs and a diverse group of 80 real-world vulnerabilities. Our study follows 
a general model of vulnerabilities and systematically compares 
the artificial vulnerabilities against real ones. In short, 
our study centers around three research questions and finds
that while artificial benchmarks attempt to approach the reality, 
they still significantly differ from the real world in several aspects. Last but 
not least, following our study, we modify LAVA-M and propose a set of
strategies towards making artificial benchmarks more realistic. 

==> prev/b-acknowledgment.tex <==
\section{Acknowledgment}

==> prev/background.tex <==
\section{Background}
Aiming to detect the similarities and differences between artificial benchmarks and real-world vulnerabilities, we choose the widely-used LAVA,
DARPA Cyber Grand Challenge, and Rode0day as the 
representative artificial works in our study. 
Both LAVA and Rode0day include similar bugs structurally, 
which injected to the standard programs. Also, the DARPA Cyber Grand Challenge contains a series of fairly small programs written by security exports with known vulnerabilities interacting with
a custom operating system.
In this section, we give background information on each of them.
% the design of LAVA, 
% especially how LAVA inserts bugs into program source code.

\subsection{LAVA}
LAVA is a prevalent ground-truth corpora generator, which 
can efficiently and automatically add potential memory safety 
errors into C/C++ programs on demand. In this way, it creates 
a huge bug corpora for tool developers and enables rigorous 
tool evaluations. LAVA currently concentrates on injecting 
out-of-bounds reading and writing bugs, and produces corresponding
proof-of-concept inputs as their triggers, rather than the
actual exploits\cite{dolan2016lava}.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{figs/LAVAOverview.pdf}
	\caption{An Overview of LAVA.}
	\label{fig:LavaOverview}   
\end{figure}

Figure~\ref{fig:LavaOverview} presents an overview of LAVA.
When LAVA obtains a program source and its series of input files,
it runs the program with dynamic taint analysis\cite{newsome2005dynamic}
on each specific input to see how each byte of the input file spreads
in the program. LAVA identifies execution trace points in the program 
where the input bytes are \emph{dead} (not used to decide any branches
up to that point), \emph{uncomplicated} (not modified), and
\emph{available} in some program variables, namely \textbf{DUAs}. 
Since DUAs are often a direct copy of input bytes and can be set 
to any chosen value without sending the program along a different 
path, LAVA intends to regard them as candidate triggers for memory
corruption.

Then, LAVA needs to find potential attack points temporally after 
a DUA along the trace to actually trigger the bug. LAVA defines
an attack point as the source code location where a DUA could 
be used to make a program vulnerable. 
For example, if the target is to inject a buffer overflow, the 
memory copy without a bound check will be a reasonable attack point. 
Similarly, if the vulnerability is an out-of-bound read, the read via 
the pointer dereference and the array index are consequent points. 
Before the DUA is made to be vulnerable, its trigger condition is
checked at the attack point, ensuring that the bug can be triggered
under controlled conditions. 

Finally, LAVA introduces a dataflow relationship between DUA and 
the attack point which occurs after the DUA in the trace. When
LAVA makes the DUA value available at the attack point, it will
meet two situations. The first one is that, if the DUA is in the 
range of the attack point, it will be directly used to cause memory
corruption at the attack point. The other is that, when the DUA is
not in scope, it will add new codes to siphon the DUA off into 
a safe place, such as a static or global data structure, then
retrieve and make use of it at the attack point. 

%% Details of inserting bugs directly/indirectly with Code Tables %%
\iffalse
As LAVA only 
injects buffer overflows into programs, we give concrete examples 
to describe the above two approaches as follows.

\begin{table}[htbp]
\centering
\begin{lstlisting}[language=c++]
void foo(int x, int y, char *c, char *s, int n)
{
    int z = x + y;
    if(x != 0xdeadbeef)
        return;
    for(int i = 0; i < n; i++)
        z += buffer[i];
    //origin source code
    strcpy(s, c, n + z);
    //bug : 
    //strcpy(s + (y == 0x6c617661) * y, c, n + c);
}
\end{lstlisting}
\caption{A bug directly inserted by LAVA. The integer {\tt y} of input is in scope at the attack point and if the input contains the correct trigger value, then an buffer overflow will occur.}
\label{tab:lava:direct}
\end{table}

\begin{itemize}
    \item  As is shown in Table~\ref{tab:lava:direct}, entering the
    function foo, the argument {\tt y} is in scope at the attack 
    point, so it can simply be used at the attack point to cause 
    the vulnerability. More specifically, {\tt y} is a direct copy 
    of input bytes and not used to decide branches as {\tt x}, 
    so it meets the requirements of DUAs and is ideal to control 
    a vulnerability. If {\tt y} is equal to the magic value, there will be a memory corruption.
    
    \item Tabel~\ref{tab:lava:indirect} shows the condition 
    when DUA is not in scope. 
    At the DUA site, LAVA adds a new call to {\tt lava\_set} to copy the DUA's value into a global variable. 
    At the attack point, {\tt lava\_get} retrieves the value and compares it to the magic value. 
    In this way, the DUA is added to the attacked pointer 
    if the condition is met, and will lead to a memory 
    corruption.
\end{itemize}


\begin{table}[htbp]
\centering
\begin{lstlisting}[language=c++]
void receive_input(int fd)
{
    ...
    read(fd, s, 100);
    lava_set(*(int *)s);
    ...
}
...
int foo(int m)
{
    int n[20];
    //original source code
    n[0] = 1;
    //bug
    //n[0 + (lava_get() == 0x6c617661) * lava_get()] = 10;
}
\end{lstlisting}
\caption{A bug indirectly inserted by LAVA. The function {\tt lava\_get} retrieves the value last stored by a call to {\tt lava\_set}. If the condition is met, a buffer overflow will occur.}
\label{tab:lava:indirect}
\end{table}

\fi


% When developers evaluate their fuzzing tools, they run it and 
% observe what it finds. Fuzzing tools usually treat the program as a 
% black box with coverage-guided tracing, and randomize individual bytes.
% According to the design of LAVA, we find that bugs inserted by LAVA
% designed to be triggered if and only if a particular set of four-byte
% input is set to a magic value, which unlikely to be discovered 
% for fuzzing tools in this way.


\subsection{DARPA Cyber Grand Challenge}

As same as LAVA dataset, the DARPA CGC, a competition among autonomous vulnerability analysis systems is a widely adopted dataset in recent studies~\cite{chen2018angora,li2017steelix,rawat2017vuzzer,zhao2019send} for evaluation. 
The benchmark can verify detected vulnerabilities by providing ground-truth. 
DARPA contains the 248 challenges with 296 binary programs, as some of the challenges includes multiple vulnerable binaries~\cite{peng2018t}, which are deliberately devised by security experts to evaluate bug finding tools. 
Each of challenge is injected one or more memory corruption vulnerabilities of various type and difficulty. 

The Cyber Grand Challenge is used under a custom operating 
system, DARPA Experimental Cyber Research Evaluation Environment (DECREE), which supports software written with a text-based 
interface to simplify analysis programs. 
The applications of Cyber Grand Challenge vary widely in complexity, such as web servers, text-based video games and so on. 
As a result, many binaries are hard to trigger because of their large input spaces and complex protocols.

Each Cyber Grand Challenge binary has a description including 
a brief summary of the program's intend written by the program authors, which usually four to five sentences. 
As for every challenge, it comes along with at least one vulnerability and proof-of-concept exploits, which make it possible to measure the effectiveness of vulnerability detection tools. 


\subsection{Rode0day}
As is mentioned above, Rode0day~\cite{Rode0dayWeb} is a monthly basis bug finding contest, which is also a benchmark to evaluate vulnerability discovery techniques. 
Rode0day challenges are all standard 32-bit Linux ELF files using automated bug insertion to generate a new corpus of buggy programs for each competition. 

Based on technology of LAVA, Rode0day modifies the data flow between DUA and Attack points by adding function arguments to 
increase complexity and remove the helper functions used artificially.
Rode0day also add a compile-time flag to the modified C-source files that can produce versions of the binaries that logged to standard output whenever a DUA guard was successfully triggered, which can easily determine which bug a competitor triggered when an input causes a crash.


\subsection{Memory corruption vulnerabilities}
Today, the most common used low-level and performance critical systems, like web browsers, web servers and operating systems are written in C/C++. 
In computer security, memory corruption vulnerabilities in software written in C or C++ are one of the oldest problems~\cite{szekeres2017memory}. 
The lack of memory safety in these languages allows bugs such as buffer overflow and use-after-free that attackers can exploit to maliciously alter the program’s behavior, and often, take full control over the entire system~\cite{checkoway2010return,bletsch2011jump,wojtczuk2001advanced}. 

